Audience Creation for Consumables -- Simple and Scalable Precision Merchandising for a Growing Marketplace

Consumable categories, such as grocery and fast-moving consumer goods, are quintessential to the growth of e-commerce marketplaces in developing countries. In this work, we present the design and implementation of a precision merchandising system, which creates audience sets from over 10 million consumers and is deployed at Flipkart Supermart, one of the largest online grocery stores in India. We employ temporal point process to model the latent periodicity and mutual-excitation in the purchase dynamics of consumables. Further, we develop a likelihood-free estimation procedure that is robust against data sparsity, censure and noise typical of a growing marketplace. Lastly, we scale the inference by quantizing the triggering kernels and exploiting sparse matrix-vector multiplication primitive available on a commercial distributed linear algebra backend. In operation spanning more than a year, we have witnessed a consistent increase in click-through rate in the range of 25-70% for banner-based merchandising in the storefront, and in the range of 12-26% for push notification-based campaigns.

==> helper/data.tex <==
\section{Dataset}
The Consumables product market of Flipkart's  spans all the major metros across India. The dataset consists of 1.58 million repeat purchasers at Flipkart Supermart who have bought products across 90 stores(a category construct at Flipkart's Supermart) ranging from Grocery, FMCG and other variety of consumable products. The dataset has 27 million total number of purchases over a time span of 15 months from January 2018 to March 2019. Each purchase is a 4-tuple having fields $<$ \textit{purchase-id}, \textit{store-path}, \textit{timestamp}, price$>$ where \textit{purchase-id} is unique identifier associated with the transaction and \textit{store-path} is a alphanumeric encoding of the path traversed by the product category in the tree-structured taxonomy $\mathcal{C}$. 

\paragraph{Tree Structured Taxonomy.} An undirected tree of 3 levels describes the hierarchy of categories of the consumable products at Flipkart with products listed below the leaf nodes as shown in Figure \textcolor{red}{xxx}. For example the category \textit{Salt} traverses the path \textit{Staples} $\mid$ \textit{Sugar, Jaggery \& Salt} $\mid$ \textit{Salt} in the taxonomy. Each node of the tree is encoded by a 3 digit alphanumeric string and \textit{store-path} for a particular item/product is the path traversed in the taxonomy by the category to which the product belongs except that each node in the path is encoded by its corresponding 3 digit alphanumeric encoding. For example \textit{Salt} is encoded as \textit{djb} and the \textit{store-path} for all items belonging to \textit{Salt} category is given by \textit{bpe} $\mid$ \textit{fdl} $\mid$ \textit{djb}. 

\subsection{Data nuances specific to Supermart}
\paragraph{Skewness} Since users considered in the dataset are repeat purchase users each user has a minimum of 2 purchases and maximum number purchases is around 1500. The distribution of purchases across users shows a power law distribution, as seen in Figure \ref{fig:acnt_dist}, it shows a large segment of the users fall in the low purchase bucket. 

\iffalse
\begin{figure}[H]
\centering
\includegraphics[width=0.50\textwidth]{fig/acnt_dist_pdf.png}
\caption{The distribution of purchases across store}
\label{fig:acnt_dist}
\end{figure}
\fi

\paragraph{Regular versus Occasional Users}
Given the skew of the distribution, we divide users into two buckets i.e., Regular, users who have made transactions on 5 months or more and Occasional, users with visits on fewer than 5 distinct months. The proportion of the head users is $\approx 8.85\%$ of the total user population but they account for $\approx 31.35\%$ of the total purchases on the platform.
The purchases across stores display the following distribution as seen in Figure \ref{fig:store_dist} where most of the store(with lower purchase) occur around the mode and few stores show higher number of transactions, indicating, bulk of the transactions are restricted to few popular stores.

\iffalse
\begin{figure}[H]
\centering
\subcaptionbox{}{\includegraphics[width=0.50\textwidth]{fig/store_dist_pdf.png}}
\includegraphics[width=0.50\textwidth]{fig/store_dist_pdf.png}
\hfill
\subcaptionbox{}{\includegraphics[width=0.50\textwidth]{fig/store_dist_cdf.png}}
\includegraphics[width=0.50\textwidth]{fig/store_dist_cdf.png}
\caption{The distribution of purchases across store}
\label{fig:store_dist}
\end{figure}
\fi 

\paragraph{Head versus Tail Stores}
Again we divide the stores into two buckets i.e., Head stores, where we see more than 350,000 purchases and the rest as Tail stores. We find around 25 stores figure as Head stores accounting for $\approx 70\%$ of the total purchases whereas rest of the $\approx 30\%$ purchases fall in the remaining 65 Tail stores. 
\paragraph{Sparseness.} 
The earlier discussion also shows the sparsity of data at the both user and store level. We examine the diversity of stores across user by checking the distribution of number of unique stores across users as shown in Figure \ref{fig:store_acnt_dist}. This makes as stronger case for data sparsity by showing not only do most of the users purchase less but their purchase only from few stores.
